CosmoPMC: Cosmology Population Monte Carlo

We present the public release of the Bayesian sampling algorithm for cosmology, CosmoPMC (Cosmology Population Monte Carlo). CosmoPMC explores the parameter space of various cosmological probes, and also provides a robust estimate of the Bayesian evidence. CosmoPMC is based on an adaptive importance sampling method called Population Monte Carlo (PMC). Various cosmology likelihood modules are implemented, and new modules can be added easily. The importance-sampling algorithm is written in C, and fully parallelised using the Message Passing Interface (MPI). Due to very little overhead, the wall-clock time required for sampling scales approximately with the number of CPUs. The CosmoPMC package contains post-processing and plotting programs, and in addition a Monte-Carlo Markov chain (MCMC) algorithm. The sampling engine is implemented in the library pmclib, and can be used independently. The software is available for download at http://www.cosmopmc.info.

==> usage_sample_from_pmcsimu.R.tex <==
\begin{verbatim}
Usage: sample_from_pmcsimu.R [options] sample [sample1 [sample2 ...]]


Options:
	-h, --help
		Show this help message and exit

	-M MULT, --mult=MULT
		Output sample MULT times input (default 1)

	-i INPUT, --input=INPUT
		Input PMC simulation file (default 'pmcsim')

	-o OUTPUT, --output=OUTPUT
		Output sample file (default 'sample')

	-s SAMPLE_METHOD, --sample_method=SAMPLE_METHOD
		(Re)sample method. 0: weighted (default), 1: residual, 2: systematic)

	--nclipw=NCLIPW
		Clip points with NCLIWP largest weights (default 0)


\end{verbatim}

